Hodge Laplacians and Hodge Diffusion Maps

We introduce Hodge Diffusion Maps, a novel manifold learning algorithm designed to analyze and extract topological information from high-dimensional data-sets. This method approximates the exterior derivative acting on differential forms, thereby providing an approximation of the Hodge Laplacian operator. Hodge Diffusion Maps extend existing non-linear dimensionality reduction techniques, including vector diffusion maps, as well as the theories behind diffusion maps and Laplacian Eigenmaps. Our approach captures higher-order topological features of the data-set by projecting it into lower-dimensional Euclidean spaces using the Hodge Laplacian. We develop a theoretical framework to estimate the approximation error of the exterior derivative, based on sample points distributed over a real manifold. Numerical experiments support and validate the proposed methodology.

==> Draft_files/appBback.tex <==
We denote by $V$ a linear subspace of dimension $m$ of $\mathbb{R}^n$.

\begin{definition}
\label{def:form2811}        
    A $k-$alternating form  $w:\underbrace{V \times V \times \cdots \times V}_{k-times} \to \mathbb{R}$ defined over a vector space $V$ is a multilinear map such that is alternating, that is, if for all vectors $v_1,v_2,\cdots,v_k$ and and any permutation $\sigma \in S_k$
    \begin{equation*}
        w(v_{\sigma(1)},\cdots,v_{\sigma(k)})=(\text{sign} \, \sigma) w(v_1,\cdots,v_k)
    \end{equation*}
\end{definition}

Similarly, we define a \( k \)-alternating array as follows:
\begin{definition}\label{def:alternatingmulti}
  A $k-$ dimensional array $ f \in \underbrace{V \otimes V \otimes \cdots \otimes V}_{k-times}$ is called \( k \)-alternating array in \( V \) if it satisfies the following condition:
\begin{itemize}
    \item \textbf{C1.}For all indices $ i_1,i_2,\cdots,i_k \in I_n$ and all permutation $\sigma \in S_k$, we have:
$f(i_{\sigma(1)},i_{\sigma(2)},\cdots,i_{\sigma(k)})=(\text{sign} \, \sigma)f(i_1,i_2,\cdots,i_k)$.
\end{itemize}
\end{definition}

We denote the set of $k-$ alternating forms as $\bigwedge^k(V)$ and the set of  $k-$ alternating arrays as $\Theta^k(V)$. An important property is that any $k-$ dimensional array $f \in \underbrace{V \otimes \cdots \otimes V}_{k \text{-times}}$, even if it is not alternating, satisfies the following property, whose proof is straightforward

\begin{pro} \label{propiedad:alternante}
For every permutation $\sigma \in S_{k}$, we let $f^{\sigma}(i_1, \cdots, i_{k}):=f(i_{\sigma(1)}, \cdots, i_{\sigma(k)})$, then for any vectors  $v_1,\cdots, v_k \in V$ we have:
\begin{equation*}
     <f^{\sigma}, v_1 \otimes v_2 \cdots \otimes v_{k}>_{F}=<f,v_{\sigma(1)} \otimes v_{\sigma(2) } \cdots \otimes v_{\sigma(k)} >_{F}
\end{equation*} 
\end{pro}
The first question is how to associate each alternating form with an $k-$ alternating array. The following result answers this question, using the universal property of the tensor product as the main idea.

\begin{prop}
\label{proposicion:universal}
    Let $V$ a $m-$ dimensional linear subspace of $\mathbb{R}^n$ and $w \in \bigwedge^k(V) $ an alternating $k-$ form. Then, there exists an unique $k-$ alternating array $W \in \Theta^k(V)$ such that:
    \begin{equation}\label{eq:tensorproductoexistencia}
        w(v_1,v_2,\cdots,v_k)= < W, v_1 \otimes v_2 \cdots \otimes v_k>_{F}
    \end{equation} 
    where $< \cdot , \cdot>$ is the Frobenius inner product for arrays defined as in \cref{productointernoarreglos}.
\end{prop}

\begin{proof}
The Universal theorem (Proposition 12.7 of \cite{lee2012introduction} p.309) says that there exists a unique linear map $L: V \otimes \cdots \otimes V \to \mathbb{R}$ such that the following diagram commutes
\begin{figure}[H]
\centering
\includegraphics[width=.41\textwidth]{teoremauniversal.JPG}
\caption{Commutative diagram for the functions $w$, $L$ and $\pi$.}
\label{fig:teoremauniversal}
\end{figure}
where $\pi:\underbrace{V \times \cdots \times V}_{k-times} \to \underbrace{V \otimes \cdots \otimes V}_{k-times}$ is given by $\pi(v_1,\cdots,v_k)=v_1\otimes \cdots \otimes v_k$. The Riesz representation theorem guarantees that there exists a unique $k-$ dimensional array $W \in \underbrace{V \otimes \cdots \otimes V}_{k-times}$ such that $L(v_1 \otimes v_2 \cdots \otimes v_k)=<W,v_1 \otimes v_2 \cdots \otimes v_k>_{F}$  for all $v_1,v_2, \cdots, v_k \in V $ and this together with the commutative diagram proves Eq. \eqref{eq:tensorproductoexistencia}. To show that $W$ is alternating, let $\sigma \in S_k$ a permutation and consider the form $w^\sigma$ as in \cref{propiedad:alternante}, then by the same property:
\begin{equation*}
\begin{array}{rcl}
     <W^{\sigma}, v_1 \otimes v_2 \cdots \otimes v_{k}>_{F}&=&<W,v_{\sigma(1)} \otimes v_{\sigma(2) } \cdots \otimes v_{\sigma(k)} >_{F}\\
     \, & = & w(v_{\sigma(1)}, v_{\sigma(2) }, \cdots ,v_{\sigma(k)}) \\
    \, & =  &(\text{sgn} \, \sigma) w(v_1,\cdots,v_k)
     \end{array}
\end{equation*}
Observe that $W^\sigma \in \underbrace{V \otimes \cdots \otimes V}_{k-times}$, then, the uniqueness of $W$ guarantees that $(\text{sgn} \, \sigma) W^{\sigma}=W$ and this proves the claim.
\end{proof}

\begin{examp}
    As example to illustrate the previous theorem consider the determinant  as alternating form over $\R^n$, then for any vector $v_1,v_2, \cdots, v_n$,
    \begin{equation*}
    \begin{array}{rcl}
        \det(v_1,v_2, \cdots, v_n) & = & \sum_{\sigma \in S_k} (\text{sgn} \, \sigma) v_{1}(\sigma(1)) \cdots v_{n}(\sigma(1)) \\
        \, & = & < W, v_1 \otimes v_2 \cdots \otimes v_n>_{F} \\
         \end{array}
    \end{equation*}
where the matrix $W(i_1, \cdots,i_n)$ is defined as $\text{sgn} \, \sigma $ if there exist a permutation $\sigma $ with $\sigma(s)=i_s$ for $1\le s \le n$ and $0$ otherwise. In the two dimensional case $\R^2$ the $k-$ alternating array $W$ is given by
 $$\begin{pmatrix}
  0 & 1\\ 
  -1 & 0
\end{pmatrix}.$$  
\end{examp}
\begin{rem}\label{remarkisomorfismo}The previous proposition allows to define an isomorphism $I$ between alternating forms $\bigwedge^k(V)$ and $k-$ alternating arrays $\Theta^k(V)$ as $I: \bigwedge^k(V) \to \Theta^k(V)$ such that $I(w)=W$, where $W$ is the $k-$ dimensional array given by Proposition \ref{proposicion:universal}.
\end{rem}



\begin{rem}\label{observacionprojectionalternada}
    Given an alternating form $w \in \bigwedge^k(\R^n)$ and a linear subspace $V$ of $\R^n$, the restriction $w |_{V \times \cdots V}$ induces an alternating form in $\bigwedge^k(V)$. In this case, it is straightforward to show that $I(w |_{V \times \cdots V})= \mathcal{P}_{V \otimes \cdots \otimes V}(I(w))$, where $\mathcal{P}_{V \otimes \cdots \otimes V}$ is the orthogonal projection onto the subspace $V \otimes \cdots \otimes V$. Therefore for any $k-$ alternating array $M \in \Theta^k(\R^n)$ the projection onto the tensor space ${V \otimes \cdots \otimes V}$ induces an $k-$ alternating array on the linear subspace $V$, which is given by, $\mathcal{P}_{V \otimes \cdots \otimes V}(M) \in \Theta^k(V)$.
 \end{rem}

In the similar way that it was defined for alternating forms, as in Property \ref{propiedad:alternante}, for any permutation $\sigma$ and for any $k-$ dimensional array $W$, we define $W^{\sigma}$ as $W^{\sigma}(v_1,\cdots,v_k)=(\text{sgn} \, \sigma)W(v_{\sigma(1)},\cdots,v_{\sigma(k)})$ \textcolor{red}{esto no coincide con la def? dada en Property 1} and the tensor product of two multilinear forms as 
 \begin{equation*}
     (w_1 \otimes w_2)(u,v)=w_1(u) w_2(v)
 \end{equation*}


Now, we define the wedge product for alternating forms and $k-$ dimensional arrays, and we show that both definitions are equivalents.
 Let $w_1$ and $w_2$ be two alternating forms (respectively  alternating arrays) of dimensions $k_1$ and $k_2$, we define the wedge product $w_1 \wedge w_2 $ as

\begin{equation*}
    w_1 \wedge w_2=\frac{1}{k_1! k_2!} \sum_{\sigma \in S_{k_1+k_2}} (\text{sgn} \, \sigma) (w_1 \otimes w_2)^{\sigma} 
\end{equation*}


\begin{prop}
\label{isobundles}
Let $w_1 \in \Lambda^{k_1}(V) $ and $w_2 \in \Lambda^{k_2}(V)$ then:

\begin{equation*}
    I(w_1 \wedge w_2)=I(w_1) \wedge I(w_2)
\end{equation*}
    
\end{prop}

\begin{proof}
  Observe that for all $v_1,\cdots, v_{k_1}, v_{k_1+1}, \cdots, v_{k_1+k_2} \in V$, then by Property \ref{propiedad:alternante}

    \begin{equation*}
    \begin{split}
        <I(w_1) \wedge I(w_2), v_1\otimes \cdots \otimes v_{k_1} \otimes v_{k_1+1} \otimes \cdots \otimes v_{k_1+k_2}>_{F}\\
        = \frac{1}{k_1! k_2!} \sum_{\sigma \in S_{k_1+k_2}} (\text{sgn} \, \sigma) <I(w_1) \otimes I(w_2), v_{\sigma (1)}\otimes \cdots \otimes v_{\sigma (k_1)} \otimes v_{\sigma (k_1+1)} \otimes \cdots \otimes v_{\sigma (k_1+k_2)}>_{F}
    \end{split}
    \end{equation*}

    \begin{equation*}
       = \frac{1}{k_1! k_2!} \sum_{\sigma \in S_{k_1+k_2}} (\text{sgn} \, \sigma) <I(w_1) \otimes I(w_2), v_{\sigma (1)}\otimes \cdots \otimes v_{\sigma (k_1)} \otimes v_{\sigma (k_1+1)} \otimes \cdots \otimes v_{\sigma (k_1+k_2)}>_{F}
    \end{equation*}

        \begin{equation*}
       = \frac{1}{k_1! k_2!} \sum_{\sigma \in S_{k_1+k_2}} (\text{sgn} \, \sigma) <I(w_1) , v_{\sigma (1)}\otimes \cdots \otimes v_{\sigma (k_1)} >   < I(w_2),  v_{\sigma (k_1+1)} \otimes \cdots \otimes v_{\sigma (k_1+k_2)}>_{F}
    \end{equation*}  

           \begin{equation*}
       =  \frac{1}{k_1! k_2!} \sum_{\sigma \in S_{k_1+k_2}} (\text{sgn} \, \sigma) (w_1 \otimes w_2)^{\sigma} ( v_{1}, \cdots , v_{k_1} , v_{k_1+1} , \cdots , v_{k_1+k_2})
    \end{equation*}  

              \begin{equation*}
       = (w_1 \wedge w_2) (v_1,\cdots, v_{k_1}, v_{k_1+1}, \cdots, v_{k_1+k_2})
    \end{equation*}  
Since $I(w_1) \wedge I(w_2)$ is in $\Theta^{k_1+k_2}(V)$ the uniqueness of  Eq \eqref{eq:tensorproductoexistencia} guarantees that $I(w_1) \wedge I(w_2)= I(w_1 \wedge w_2)$. 
\end{proof}

If $w \in V$, then, we define its dual functional $w^{*} \in \bigwedge^{1}(V)$ as $w^{*} (v)=<w,v>_{F}$ for all $v\in V$, in this case $I(w^{*})=w$. In \cite{lee2012introduction}, Chapter 14, p.356, it is shown that for $v_1,\cdots, v_k, w_1,\cdots, w_k \in V$ the following identity holds:

\begin{equation*}
    w_1^{*} \wedge \cdots \wedge  w_k^{*}(v_1,\cdots,v_k)= \det(<w_i,v_j>)
\end{equation*}

\begin{equation*}
  = \sum_{\sigma \in S_{k}} (\text{sgn} \, \sigma) <w_{\sigma(1)},v_1> \cdots <w_{\sigma(k)},v_k> _{F}
\end{equation*}

\begin{equation*}
 =< \sum_{\sigma \in S_{k}}  (\text{sgn} \, \sigma) w_{\sigma(1)} \otimes \cdots \otimes w_{\sigma(k)}, v_1 \otimes \cdots \otimes v_k>_{F}
\end{equation*}

Thus, 
\begin{equation} \label{eq:expansionwedge}
    w_1 \wedge \cdots \wedge w_k= I(w_1^{*} \wedge \cdots \wedge  w_k^{*})=  \sum_{\sigma \in S_{k}}  (\text{sgn} \, \sigma) w_{\sigma(1)} \otimes \cdots \otimes w_{\sigma(k)}
\end{equation}

    
In the same way that the vector space of $k-$ dimensional arrays has an inner product structure, we give the set of alternating forms $\Lambda^{k}(V)$ \textcolor{red}{Estas confundiendo formas con $k$-vectores que son elementos de la $k$-exterior power y el producto interno en $\Lambda^{k}(V)$ es el inducido por un producto interno en $V$ previamente fijado que en nuestro caso esta dado por la metrica Riemaniana} an inner product $<\cdot,\cdot>_{\Lambda^{k}(V)}$ as follows: Let $w_1, w_2 \in \Lambda^{k}(V)$. The inner product is defined using the inner product of their images under the isomorphism $I$ as

\begin{equation*}
    <w_1,w_2>_{\Lambda^{k}(V)}=<I(w_1), I(w_2)>_{F}
\end{equation*}

Therefore the application $I:\Lambda^{k}(V) \to \Theta^{k}(V)$ is an isometric isomorphism that preserves the wedge product.
If $v_1, v_2, \cdots, v_m$ is an orthonormal basis for  $V$, then the set of wedge products
\begin{equation}
\label{wpbase}
    \llave{ \frac{1}{\sqrt{k!}}v_{i_1}^{*} \wedge v_{i_2}^{*}  \wedge \cdots \wedge v_{i_k}^{*} \mid i_1<i_2< \cdots < i_k }
\end{equation}
is an orthonormal basis for $\Lambda^{k}(V)$. In fact, for any indices $i_1<i_2< \cdots < i_k$ and $j_1<j_2< \cdots < j_k$, we have by Eq. \eqref{eq:expansionwedge}
\begin{equation*}
    <v_{i_1} ^{*} \wedge v_{i_2}  ^{*}\wedge \cdots \wedge v_{i_k} ^{*}, v_{j_1} ^{*} \wedge v_{j_2} ^{*} \wedge \cdots \wedge v_{j_k} ^{*}>_{\Lambda^{k}(V)}
\end{equation*}
\begin{equation*}
=\sum_{\sigma_1, \sigma_2 \in S_k} (\text{sgn} \, \sigma_1) (\text{sgn} \, \sigma_2) <v_{i_{\sigma_1(1)}}\otimes \cdots \otimes v_{i_{\sigma_1(k)}},v_{j_{\sigma_2(1)}}\otimes \cdots \otimes v_{j_{\sigma_2(k)}}>_{F}
\end{equation*}
\begin{equation*}
=\sum_{\sigma_1, \sigma_2 \in S_k} (\text{sgn} \, \sigma_1) (\text{sgn} \, \sigma_2) <v_{i_{\sigma_1(1)}}, v_{j_{\sigma_2(1)}}>_{F} \cdots <v_{i_{\sigma_1(k)}}, v_{j_{\sigma_2(k)}}>_{F}
\end{equation*}
From the previous equation, we conclude that if the indices \( i_1 < i_2 < \cdots < i_k \) and \( j_1 < j_2 < \cdots < j_k \) are different, then the sum consists entirely of zeros, so the inner product is zero. This shows that the wedge products \( v_{i_1} \wedge v_{i_2} \wedge \cdots \wedge v_{i_k} \) and \( v_{j_1} \wedge v_{j_2} \wedge \cdots \wedge v_{j_k} \) are orthogonal. 
When the indices are equal, i.e., \( i_l = j_l \) for all \( 1 \le l \le k \), the terms in the sum are zero unless \( \sigma_1 = \sigma_2 \), in which case the term is equal to 1. Therefore, we have:
\[
\langle v_{i_1} \wedge v_{i_2} \wedge \cdots \wedge v_{i_k}, v_{i_1} \wedge v_{i_2} \wedge \cdots \wedge v_{i_k} \rangle_{\Lambda^k(V)} = \sum_{\sigma \in S_k} 1 = k!
\]
This completes the proof.

==> Draft_files/appCguardar.tex <==
\begin{lem}
\label{lemmatangentprojection}
For each \( x \in \mathcal{M} \) and \( v \in \mathbb{R}^n \), let \(\mathcal{P}_{T_x \mathcal{M}}(v)\) be the orthogonal projection of the vector \( v \) onto the tangent space \( T_x \mathcal{M} \). For a matrix \( V \) with columns \( V = [v_1 \, v_2 \, \cdots \, v_k] \), where \( v_i \in \mathbb{R}^n \), define \(\mathcal{P}_{T_x \mathcal{M}}(V)\) as the matrix whose columns are:
\[
\mathcal{P}_{T_x \mathcal{M}}(V) = [\mathcal{P}_{T_x \mathcal{M}}(v_1) \, \mathcal{P}_{T_x \mathcal{M}}(v_2) \, \cdots \, \mathcal{P}_{T_x \mathcal{M}}(v_k)].
\] then
  
\begin{enumerate}
    \item For any matrix $V$ the map $y \to \mathcal{P}_{T_y \mathcal{M}}(V) $ is smooth for all $y \in \mathcal{M}$.
    \item The following identity holds: $\mathcal{P}_{T_y \mathcal{M}}(v)=O(y) O(y)^{T} v$ for all $v \in \R^n$
    \item If \(\det\left((\mathcal{P}_{T_y \mathcal{M}}(O(x)))^T \mathcal{P}_{T_y \mathcal{M}}(O(x))\right) \neq 0\), then the following identity holds:
   \[
   \mathcal{P}_{T_y \mathcal{M}}(O(x)) \left((\mathcal{P}_{T_y \mathcal{M}}(O(x)))^T \mathcal{P}_{T_y \mathcal{M}}(O(x))\right)^{-1/2} = O(y) O(y, x).
   \]
\end{enumerate}
\end{lem}


\begin{proof}
To prove item (1), let \((x_1, x_2, \ldots, x_d)\) be local coordinates around \(x\). Then the map \( y \mapsto \mathcal{P}_{T_y \mathcal{M}}(V) \) can be expressed as:
\[
y \mapsto \sum_{i=1}^d \langle v, \frac{\partial}{\partial y_i} \rangle \frac{\partial}{\partial y_i},
\]
which is smooth, thus proving the claim.

For item (2), note that the proof is straightforward since the columns of the matrix \( O(y) \) form an orthonormal basis.

To prove item (3), we need a suitable computation. Assume that the singular value decomposition (SVD) of \( O(y)^T O(x) \) is:
\[
O(y)^T O(x) = U_{(y,x)} \Sigma_{(y,x)} V_{(y,x)}^T.
\]

Then, using item (2):
\[
\mathcal{P}_{T_y \mathcal{M}}(O(x)) = O(y) O(y)^T O(x) = O(y) U_{(y,x)} \Sigma_{(y,x)} V_{(y,x)}^T.
\]

Let \( L_y \) be the matrix \( L_y = \mathcal{P}_{T_y \mathcal{M}}(O(x)) \). Then:
\begin{equation}
    \label{ecuacionsingpositiv}
\begin{aligned}
L_y^T L_y &= V_{(y,x)} \Sigma_{(y,x)} U_{(y,x)}^T O(y)^T O(y) U_{(y,x)} \Sigma_{(y,x)} V_{(y,x)}^T \\
&= V_{(y,x)} \Sigma_{(y,x)}^2 V_{(y,x)}^T.
\end{aligned}
\end{equation}


Since \(\det(L_y^T L_y) \neq 0\), all the singular values in the diagonal matrix \(\Sigma_{(y,x)}^2\) are positive. Therefore, the inverse of the square root of \( L_y^T L_y \) exists and is given by:
\[
(L_y^T L_y)^{-1/2} = V_{(y,x)} \Sigma_{(y,x)}^{-1} V_{(y,x)}^T.
\]

This shows that:
\[
\begin{aligned}
L_y (L_y^T L_y)^{-1/2} &= O(y) U_{(y,x)} \Sigma_{(y,x)} V_{(y,x)}^T V_{(y,x)} \Sigma_{(y,x)}^{-1} V_{(y,x)}^T \\
&= O(y) O(y,x).
\end{aligned}
\]

\end{proof}



A key step in proving Proposition \ref{prop:contructionlocalframe} is to show that the map \( X \mapsto X^{-1/2} \) is well-defined and smooth over a specific space that is a subset of the general linear group \( GL(\mathbb{R}^n) \), which includes all \( n \times n \) invertible matrices with real coefficients. This result is well-known and can be found in standard references like \cite{limaanalisevol2} (Portuguese edition). For completeness, we provide a proof here, starting with the following auxiliary lemmas:


\begin{lem} \label{lemadiff1}
Let \( f_1: GL(\mathbb{R}^n) \to GL(\mathbb{R}^n) \) be the function defined by \( f_1(X) = X^{-1} \). This function is a diffeomorphism on the set of invertible matrices \( GL(\mathbb{R}^n) \).
\end{lem}


\begin{proof}
    First, we prove that $f_1$ defines a diffeomorphism. It is clear that $f_1$ is a bijection, in addition, since the determinant is a continuous function then for $A \in GL(\R^n)$ and $V$ any $n \times n$ matrix and $h$ a small real number, it satisfies $A+hV \in GL(\R^n)$ then by the geometric series
    \begin{equation*}
    \begin{array}{rcl} 
        (A+h V)^{-1}& = & A^{-1} (Id+h VA^{-1})^{-1} \\
        & = &A^{-1} (Id- h VA^{-1} +\sum_{i=2}^{\infty} (-1)^i h^{i} (VA^{-1})^i)\\
        & = & A^{-1} -h A^{-1} V A^{-1} + O(h^2))
        \end{array}
    \end{equation*}
And this proves that $f_1$ is differentiable with $Df_1(A)(V)=-A^{-1} V A^{-1}$, moreover since $(f_1)^{-1}=f_1$, then $f_!$ is a diffeomorphism.
\end{proof}

On the other hand, let \( SP(\mathbb{R}^d) \subseteq GL(\mathbb{R}^n)  \) represent the space of symmetric and positive-definite matrices. The square root function is smooth on this space and defines a diffeomorphism.

\begin{lem}\label{lemadiff2}
    The map \( f_2: SP(\mathbb{R}^d) \to SP(\mathbb{R}^d) \), defined by \( f_2(X) = X^2 \), is a diffeomorphism.
\end{lem}

By Theorem 13 on page 341 of \cite{hoffman1971linear}, the map \( f_2 \) is a bijection. Moreover, for any \( A \in SP(\mathbb{R}^d) \), square matrix \( V \), and small real number \( h \):

\[
(A + hV)^2 = A^2 + h (AV + VA) + h^2 V^2,
\]

which implies that \( Df_2(A)(V) = AV + VA \). We claim that this derivative is injective. If \( Df_2(A)(V) = 0 \), then \( AV = -VA \). Let \( (\lambda, e) \) be an eigenpair of \( A \), then:

\[
A(V(e)) = V(A(e)) = -\lambda V(e).
\]

Since \( A \) has positive eigenvalues, \( V(e) \) must be zero; otherwise, \( (-\lambda, V(e)) \) would be an eigenpair, implying that both \( \lambda \) and \( -\lambda \) are eigenvalues of \( A \), which contradicts the positivity of the eigenvalues. As \( V(e) = 0 \) for all eigenvectors of \( A \), it follows that \( V = 0 \), proving that \( Df_2(A) \) is injective. By the inverse function theorem, this shows that \( f_2 \) is indeed a diffeomorphism

\,
\,
\,

\begin{proof}[Proof of Proposition \ref{prop:contructionlocalframe}]


For a fixed \( x \in \mathcal{M} \), by Item 1 of Lemma \ref{lemmatangentprojection}, the map \( y \mapsto \mathcal{P}_{T_y \mathcal{M}}(O(x)) \) is smooth over the manifold \( \mathcal{M} \). Now, by Lemmas \ref{lemadiff1} and \ref{lemadiff2}, the function
\[
    X \mapsto f_1(f_2^{-1}(X)) = X^{-1/2}
\]
is smooth over the set of positive definite matrices \( SP(\mathbb{R}^d) \). By Item 3 of Lemma \ref{lemmatangentprojection}, we have
\[
   \mathcal{P}_{T_y \mathcal{M}}(O(x)) \left((\mathcal{P}_{T_y \mathcal{M}}(O(x)))^T \mathcal{P}_{T_y \mathcal{M}}(O(x))\right)^{-1/2} = O(y) O(y, x).
\]
Since the map \( y \mapsto \mathcal{P}_{T_y \mathcal{M}}(O(x)) \) is smooth by Item 1 of Lemma \ref{lemmatangentprojection}, and by Equation \eqref{ecuacionsingpositiv} of the same Lemma, the matrix
\[
    (\mathcal{P}_{T_y \mathcal{M}}(O(x)))^T \mathcal{P}_{T_y \mathcal{M}}(O(x))
\]
is positive definite if and only if its determinant is non-zero. Furthermore, from Equation \eqref{ecuacionsingpositiv}, we have:
\[
   \det((\mathcal{P}_{T_y \mathcal{M}}(O(x)))^T \mathcal{P}_{T_y \mathcal{M}}(O(x))) = \det(O(y,x))^2.
\]
Thus, \(\det((\mathcal{P}_{T_y \mathcal{M}}(O(x)))^T \mathcal{P}_{T_y \mathcal{M}}(O(x))) \neq 0\) if and only if \(\det(O(y,x)) \neq 0\). Therefore, the map
\[
    y \mapsto O(y) O(y, x)
\]
is smooth in the neighborhood of \( x \) defined by \( U = \{ y \mid \det(O(y,x)) \neq 0 \} \), which is an open set since \( y \mapsto \mathcal{P}_{T_y \mathcal{M}}(O(x)) \) is smooth.

\end{proof}


==> Draft_files/appDguardar.tex <==
\begin{proof}[Proof of Lemma \ref{lemaprinformas}]

%%%%%%%New part
First, note that each function \(\phi_s\) defines a bump function over \(U(x_s, r)\). Therefore, \(\overline{\phi_s}\) is smooth over the manifold $\mathcal{M}$ and well-defined, as the sum \(\sum_{s=1}^N \phi_s\) is always positive on the set
\begin{equation*}
   U_{set}= \bigcup_{s=1}^N U(x_s, r).
\end{equation*}
 Furthermore, \(\overline{\phi_s}  \overline{h_s}\) defines a smooth function over the entire manifold \(\mathcal{M}\).\\
For item (1), note that since the functions $\overline{h_s}$ and $\overline{\phi_s}$ are bounded and the exponential function is smooth, the Lebesgue dominated convergence theorem ensures that the functions
   \begin{equation*}
      x \to \int_{\mathcal{M}} e^{\frac{-\| y-x \|^2}{2 t^2}} \sum_{s=1}^N \overline{\phi_s}(y) \overline{h_s}(y)(n_1, \cdots,n_k) q(y)dVol(y)
   \end{equation*}
and $d_t$ are smooth. Moreover, for any point $x$ on the manifold, and a smooth local orthonormal frame $v^{x}_1, v^{x}_2, \dots, v^{x}_d$ defined on the neighborhood $U(x, r)$, the orthogonal projection of the integral above can be locally written as
\begin{equation*}
    z \to \sum_{J} < \int_{\mathcal{M}} e^{\frac{-\| y-z \|^2}{2 t^2}} \sum_{s=1}^N  \overline{\phi_s}(y)  \overline{h_s}(y)  q(y) dVol(y),v^{x}_J(z)>_{F} v^{x}_J(z) 
\end{equation*}

which is smooth since the integral is smooth. Note that \(d_t(x) > 0\) and is never zero, as the exponential does not vanish in a neighborhood of \(x\). 



To prove item (2), we use similar ideas as in the proof of Theorem \ref{teoremaprincipal}. First, note that the set of multidimensional arrays can be viewed as a subspace of Euclidean space. Specifically, for all \( x \) on the manifold, we have \( \Theta^k(T_x \mathcal{M}) \subseteq \mathbb{R}^{n^k} \). Additionally, observe that for \( x \in U_{\text{set}} \):

\begin{equation}
\label{eqlocalcompu}
\begin{array}{rcl} 
 \sum_{s=1}^N \overline{\phi_s}(x) \overline{h_s}(x) &=& \sum_{x \in U(x_s, r)}^N \sum_{J} \overline{\phi_s}(x) f^{x_s}_{J}(x) v^{x_s}_{J}(x) \\
 &=& \sum_{x \in U(x_s, r)} \overline{\phi_s}(x) \sum_{J} \langle W(x), v^{x_s}_{J}(x) \rangle_{F} \, v^{x_s}_{J}(x) \\
 &=& W(x) \sum_{x \in U(x_s, r)} \overline{\phi_s}(x) \\
 &=& W(x)
 \end{array}
\end{equation}

where the sum on the right (\( \sum_{x \in U(x_s, r)} \)) is over all indices \( s \) such that \( x \in U(x_s, r) \). The last equality holds because the set \( \{v^{x_s}_{J}(x)\}_{J} \) forms an orthonormal basis for the space of multidimensional arrays.

Next, we apply Lemma \ref{lemcalculosimple} to the function \( h(y) = \sum_{s=1}^N \overline{\phi_s}(y) \overline{h_s}(y) q(y) \), along with Equation \eqref{eqlocalcompu}, to obtain:

\begin{equation*}
\begin{array}{rcl}
   \int_{\mathcal{M}} e^{-\frac{\| y - x \|^2}{2 t^2}} h(y) \, d\text{Vol}(y) & = & \int_{\mathcal{M}} e^{-\frac{\| y - x \|^2}{2 t^2}} \sum_{x \in U(x_s, r)}
 \overline{\phi_s}(y) \overline{h_s}(y) q(y) \, d\text{Vol}(y) \\
   & = & (2 \pi)^{\frac{d}{2}} t^d \sum_{x \in U(x_s, r)} \overline{\phi_s}(x) \overline{h_s}(x) q(x) \\
   & + & O(t^{d + 4\delta - 2}) + O(t^{2(1 - \delta)(d + 2)}) \\
    & = & (2 \pi)^{\frac{d}{2}} t^d W(x) q(x) + O(t^{d + 4\delta - 2}) + O(t^{2(1 - \delta)(d + 2)}).
\end{array}
\end{equation*}

Note that the error terms in the equation above are independent of \( N \), as the upper bounds for the function \( h \) and its derivatives do not depend on \( N \). In fact, by Equation \eqref{eqlocalcompu}, we have \( h(x) = W(x) q(x) \) over \( U_{\text{set}} \), which is independent of the parameter \( N \). Additionally, by Lemma \ref{lemanor}:
\begin{equation*}
   d_t(x)= (2 \pi)^{\frac{d}{2}} t^d q(x)+O(t^{d+4 \delta -2})+O (t^{2(1-\delta)(d+2)})
\end{equation*}
Thus, by combining the previous equations, we conclude that the operator \( L^{(t)}(x) \) can be expanded as:
\begin{equation*}
\begin{array}{rcl}
   L^{(t)}(x)&= & W(x)+ O(t^{d+4 \delta -2})+O (t^{2(1-\delta)(d+2)}) \\
\end{array}
\end{equation*}
\end{proof}

==> Draft_files/complete_ref.tex <==
@book{lee2012introduction,
  title={Introduction to Smooth Manifolds},
  author={Lee, J.},
  series={Graduate Texts in Mathematics},
  year={2012},
  publisher={Springer New York}
}




@ARTICLE{10227282,
  author={Gomez, Alvaro Almeida and Neto, Antônio J. Silva and Zubelli, Jorge P.},
  journal={IEEE Access}, 
  title={A Diffusion-Map-Based Algorithm for Gradient Computation on Manifolds and Applications}, 
  year={2023},
  volume={11},
  number={},
  pages={90622-90640},
  doi={10.1109/ACCESS.2023.3307772}}
 
 @book{conway_a._bannai_1993, place={New York}, title={Sphere packings, lattices and groups}, publisher={Springer-Verlag}, author={Conway, J. H. and A., Sloane N J and Bannai, E.}, year={1993}} 

@misc{cohn2022,
  doi = {10.48550/ARXIV.2206.15373},
  
  url = {https://arxiv.org/abs/2206.15373},
  
  author = {Cohn, Henry and de Laat, David and Salmon, Andrew},
  
  keywords = {Metric Geometry (math.MG), FOS: Mathematics, FOS: Mathematics},
  
  title = {Three-point bounds for sphere packing},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@Article{GLZ2018,
 Author = {Gobet, Emmanuel and Liu, Gang and Zubelli, Jorge P.},
 Title = {A nonintrusive stratified resampler for regression {Monte} {Carlo}: application to solving nonlinear equations},
 FJournal = {SIAM Journal on Numerical Analysis},
 Journal = {SIAM J. Numer. Anal.},
 ISSN = {0036-1429},
 Volume = {56},
 Number = {1},
 Pages = {50--77},
 Year = {2018},
 Language = {English},
 DOI = {10.1137/16M1066865},
 Keywords = {65C05,60H10,62G08},
 zbMATH = {6826854},
 Zbl = {1392.65011}
}


@article{muksa,
author = {Mukherjee, Sayan and Wu, Qiang and Zhou, Ding-Xuan},
year = {2010},
month = {02},
pages = {},
title = {Learning gradients on manifolds},
volume = {16},
journal = {Bernoulli},
doi = {10.3150/09-BEJ206}
}

@book{sato,
  title={Riemannian Optimization and Its Applications},
  author={Sato, Hiroyuki},
  year={2021},
  publisher={Springer}
}


@book{bloch,
  title={Hamiltonian and gradient flows, algorithms and control},
  author={Bloch, A.},
  volume={3},
  year={1994},
  publisher={American Mathematical Soc.}
}


@article{smith,
  title={Optimization Techniques on Riemannian Manifolds},
  author={S.T. Smith},
  journal={ArXiv},
  year={2014},
  volume={abs/1407.5965}
}


@article{edelman,
  title={The Geometry of Algorithms with Orthogonality Constraints},
  author={A. Edelman and Tom{\'a}s A. Arias and S.T. Smith},
  journal={SIAM J. Matrix Anal. Appl.},
  year={1998},
  volume={20},
  pages={303-353}
}


@article{yuan,
  title={Damped Newton’s method on Riemannian manifolds},
  author={M. A. A. Bortoloti and Teles A. Fernandes and O. Pereira Ferreira and J. Yuan},
  journal={Journal of Global Optimization},
  year={2020},
  volume={77},
}


@article{benarsvaiter,
  title={A steepest descent method for vector optimization},
  author={L. Mauricio Gra{\~n}a Drummond and B. F. Svaiter},
  journal={Journal of Computational and Applied Mathematics},
  year={2005},
  volume={175},
  pages={395-414}
}


@article{shub2,
  title={Newton's method on Riemannian manifolds and a geometric model for the human spine},
  author={R. L. Adler and J.P. Dedieu and J. Y. Margulies and M. Martens and M. Shub},
  journal={Ima Journal of Numerical Analysis},
  year={2002},
}


@article{shub,
  title={Complexity of B{\'e}zout’s theorem. I. Geometric aspects},
  author={M. Shub and S. Smale},
  journal={Journal of the American Mathematical Society},
  year={1993},
}


@inproceedings{smale,
  title={Newton’s Method Estimates from Data at One Point},
  author={S. Smale},
  year={1986},
  booktitle={The Merging of Disciplines: New Directions in Pure, Applied, and Computational Mathematics},
publisher={Springer New York},
}

@book{xavierdua,
  title={Fourier Analysis},
  author={Zuazo, J.D.},
  year={2001},
  publisher={American Mathematical Soc.}
}



@book{kato1995perturbation,
  title={Perturbation Theory for Linear Operators},
  author={Kato, T.},
  year={1995},
  publisher={Springer Berlin Heidelberg}
}



@book{natterer,
  title={The Mathematics of Computerized Tomography},
  author={Natterer, F.},
  year={2001},
  publisher={Society for Industrial and Applied Mathematics}
}







@book{minkowsk,
  title={The Geometry of Numbers},
  author={Olds, C.D. and Lax, A. and Davidoff, G.P. and Davidoff, G.},
  year={2000},
  publisher={Mathematical Association of America}
}






@book{MacKay2003,
  author = {MacKay, David J. C.},
  publisher = {Cambridge University Press},
  title = {Information Theory, Inference, and Learning Algorithms},
  year = 2003
}






@book{jolliffe2002principal,
  title={Principal Component Analysis},
  author={Jolliffe, I.T},
  isbn={9780387954424},
  url={https://books.google.ae/books?id=\_olByCrhjwIC},
  year={2002},
  publisher={Springer}
}




@article{Chen2014BigDA,
  title={Big Data: A Survey},
  author={M. Chen and S. Mao and Y. Liu},
  journal={Mobile Networks and Applications},
  year={2014},
  volume={19},
  pages={171-209}
}


@book{kepner2018mathematics,
  title={Mathematics of Big Data: Spreadsheets, Databases, Matrices, and Graphs},
  author={Kepner, J. and Jananthan, H. and Leiserson, C.E.},
  isbn={9780262038393},
  lccn={2017057054},
  series={MIT Lincoln Laboratory Series},
  url={https://books.google.ae/books?id=Pq9GswEACAAJ},
  year={2018},
  publisher={MIT Press}
}



@article{motipa1,
author = {Wang, Lidong and Alexander, Cheryl},
year = {2019},
month = {02},
pages = {17-26},
title = {Big Data Analytics in Healthcare Systems},
volume = {4},
journal = {International Journal of Mathematical, Engineering and Management Sciences},
doi = {10.33889/IJMEMS.2019.4.1-002}
}




article{refboug,
	author = {{ T. Bourgeron} and { C. Conca} and { R. Lecaros}},
	title = {Determining the distribution of ion channels from experimental data},
	DOI= "10.1051/m2an/2017062",
	url= "https://doi.org/10.1051/m2an/2017062",
	journal = {ESAIM: M2AN},
	year = 2018,
	volume = 52,
	number = 5,
	pages = "2083-2107",
}





@article{doumic2020,
title = {Estimating the division rate from indirect measurements of single cells},
journal = {Discrete and Continuous Dynamical Systems - B},
volume = {25},
number = {10},
pages = {3931-3961},
year = {2020},
author = {{M. Doumic} and {A. Olivier} and {L. Robert}},
}

@article{nonconserva,
title = {A note on mass-conserving solutions to the coagulation-fragmentation equation by using non-conservative approximation},
journal = {Kinetic and Related Models},
volume = {11},
number = {5},
pages = {1125-1138},
year = {2018},
author = {P. Barik, A. Giri},
}


@article{noconsevaorig,
author = {Filbet, Francis and Laurençot, Philippe},
year = {2004},
month = {12},
pages = {558-567},
title = {Mass-conserving solutions and non-conservative approximation to the Smoluchowski coagulation equation},
volume = {83},
journal = {Archiv der Mathematik},
doi = {10.1007/s00013-004-1060-9}
}






@article{nonpara,
author = {Hoang, V. Ngoc, T. Mai and Rivoirard, Vincent and Tran, V. Chi},
title = {Nonparametric estimation of the fragmentation kernel based on a partial differential equation stationary distribution approximation},
journal = {Scandinavian Journal of Statistics},
keywords = {cell division, deconvolution, growth-fragmentation, kernel rule, nonparametric estimation},
doi = {https://doi.org/10.1111/sjos.12504},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/sjos.12504},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1111/sjos.12504},
abstract = {Abstract We consider a stochastic individual-based model in continuous time to describe a size-structured population for cell divisions. This model is motivated by the detection of cellular aging in biology. We here address the problem of nonparametric estimation of the kernel ruling the divisions based on the eigenvalue problem related to the asymptotic behavior in large population. This inverse problem involves a multiplicative deconvolution operator. Using Fourier techniques we derive a nonparametric estimator whose consistency is studied. The main difficulty comes from the nonstandard equations connecting the Fourier transforms of the kernel and the parameters of the model. A numerical study is carried out and we pay special attention to the derivation of bandwidths by using resampling.}
}





@article{laurent,
author = "Laurençot, Philippe and Perthame, Benoit",
fjournal = "Communications in Mathematical Sciences",
journal = "Commun. Math. Sci.",
month = "06",
number = "2",
pages = "503--510",
publisher = "International Press of Boston",
title = "Exponential decay for the growth-fragmentation/cell-division equations",
url = "https://projecteuclid.org:443/euclid.cms/1243443992",
volume = "7",
year = "2009"
}


@book{lion,
  title={M{\'e}thode de quasi-r{\'e}versibilit{\'e} et applications},
  author={Lattès, R. and Lions, J.-L},
  lccn={68084549},
  series={Travaux et recherches math{\'e}matiques},
  url={https://books.google.com.co/books?id=F9yxAAAAIAAJ},
  year={1967},
  publisher={Dunod}
}


@article{pezu,
	doi = {10.1088/0266-5611/23/3/012},
	url = {https://doi.org/10.1088/0266-5611/23/3/012},
	year = 2007,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {23},
	number = {3},
	pages = {1037--1052},
	author = {Benoit Perthame and Jorge P Zubelli},
	title = {On the inverse problem for a size-structured population model},
	journal = {Inverse Problems},
	abstract = {We consider a size-structured model for cell division and address the question of determining the division (birth) rate from the measured stable size distribution of the population. We formulate such a question as an inverse problem for an integro-differential equation posed on the half line. We develop firstly a regular dependence theory for the solution in terms of the coefficients and, secondly, a novel regularization technique for tackling this inverse problem which takes into account the specific nature of the equation. Our results also rely on generalized relative entropy estimates and related Poincaré inequalities.}
}

@book{reguinvlib,
  title={Regularization of Inverse Problems},
  author={Engl, Heinz and Hanke, Martin and Neubauer, Andreas},
  isbn={9780792341574},
  lccn={lc96028672},
  series={Mathematics and Its Applications},
  url={https://books.google.com.co/books?id=2bzgmMv5EVcC},
  year={1996},
  publisher={Springer Netherlands}
}


@book{rud,
  title={Fourier Analysis on Groups},
  author={Rudin, Walter.},
  isbn={9780471523642},
  lccn={62012211},
  series={Wiley Classics Library},
  url={https://books.google.com.co/books?id=WlzLFUo0VzYC},
  year={1990},
}
@article{doti,
author = {Doumic, Marie and Tine, Léon},
year = {2012},
month = {06},
pages = {},
title = {Estimating the Division Rate for the Growth-Fragmentation Equation},
volume = {67},
journal = {Journal of mathematical biology},
doi = {10.1007/s00285-012-0553-6}
}


@article{pery1,
title = {Exponential decay for the fragmentation or cell-division equation},
journal = {Journal of Differential Equations},
volume = {210},
number = {1},
pages = {155-177},
year = {2005},
issn = {0022-0396},
doi = {https://doi.org/10.1016/j.jde.2004.10.018},
url = {https://www.sciencedirect.com/science/article/pii/S0022039604004231},
author = {Benoît Perthame and Lenya Ryzhik},
keywords = {Cell division, Fragmentation, Asymptotic stability},
abstract = {We consider a classical integro-differential equation that arises in various applications as a model for cell-division or fragmentation. In biology, it describes the evolution of the density of cells that grow and divide. We prove the existence of a stable steady distribution (first positive eigenvector) under general assumptions in the variable coefficients case. We also prove the exponential convergence, for large times, of solutions toward such a steady state.}
}

@article{mimipe,
title = {General entropy equations for structured population models and scattering},
journal = {Comptes Rendus Mathematique},
volume = {338},
number = {9},
pages = {697-702},
year = {2004},
issn = {1631-073X},
doi = {https://doi.org/10.1016/j.crma.2004.03.006},
url = {https://www.sciencedirect.com/science/article/pii/S1631073X04001177},
author = {Philippe Michel and Stéphane Mischler and Beno\^it Perthame},
abstract = {We consider several structured population models (age structured, size structured, maturity structured) and the general scattering equation. These models are not conservation laws, nevertheless, we show that they admit a common relative entropy structure which uses the first eigenelements of the problem. In case of scattering, it is more general than the usual ‘detailed balance principle’. Three types of consequences are deduced from this entropy structure: a priori bounds, large time convergence to the steady state and in some cases, exponential rates of convergence. To cite this article: P. Michel et al., C. R. Acad. Sci. Paris, Ser. I 338 (2004).
Résumé
Nous considérons divers modèles de populations structurées (en âge, en taille ou en maturité) et aussi l'équation de scattering. Ces modèles ne sont pas conservatifs, néammoins nous montrons qu'ils vérifient tous une structure d'entropie relative commune qui utilise les premiers éléments propres du problème et qui, dans le cas du scattering, généralise le « principe d'équilibre en détail » habituel. Trois types de conséquences découlent de cette structure entropique : des estimations a priori, la convergence en temps grand vers un état stationnaire et parfois des taux exponentiels de convergence. Pour citer cet article : P. Michel et al., C. R. Acad. Sci. Paris, Ser. I 338 (2004).}
}

@book{celdi1,
  title={Transport Equations in Biology},
  author={Perthame, Benoit.},
  isbn={9783764378424},
  lccn={2006934214},
  series={Frontiers in Mathematics},
  url={https://books.google.fr/books?id=1vZlBfhCEgMC},
  year={2006},
  publisher={Birkh{\"a}user Basel}
}



@InProceedings{celdi2,
author="Metz, Johan A.
and Diekmann, Odo.",
editor="Metz, Johan A.
and Diekmann, Odo.",
title="Formulating Models for Structured Populations",
booktitle="The Dynamics of Physiologically Structured Populations",
year="1986",
publisher="Springer Berlin Heidelberg",
pages="78--135",
abstract="By now the examples from chapter I and/or the subsequent theoretical elaboration in chapter 11 shou,ld have given you a taste lor structured population models. In this chapter we shall develop a do-it-yoursell kit enabling you to build models incorporating various amounts of biological detail.",
isbn="978-3-662-13159-6"
}


@article{celdi3,
author = {Basse, Britta and Baguley, Bruce and Marshall, Elaine and Joseph, Wayne and van Brunt, Bruce and Wake, Graeme and Wall, David},
year = {2003},
month = {11},
pages = {295-312},
title = {A mathematical model for analysis of the cell cycle in cell lines derived from human tumors},
volume = {47},
journal = {Journal of mathematical biology},
doi = {10.1007/s00285-003-0203-0}
}


@article{propol1,
author = {Greer, Meredith and Pujo-Menjouet, Laurent and Webb , Glenn},
year = {2006},
month = {11},
pages = {598-606},
title = {A mathematical analysis of the dynamics of prion proliferation},
volume = {242},
journal = {Journal of theoretical biology},
doi = {10.1016/j.jtbi.2006.04.010}
}

@article{teleco,
author = {Baccelli, François and McDonald, David and Reynier, Julien},
year = {2002},
month = {09},
pages = {77-97},
title = {A mean-field model for multiple TCP connections through a buffer implementing RED},
volume = {49},
journal = {Performance Evaluation},
doi = {10.1016/S0166-5316(02)00136-0}
}

@article{doga,
author = {Doumic, Marie and Gabriel, Pierre},
year = {2009},
month = {07},
pages = {757-783},
title = {Eigenelements of a General Aggregation-Fragmentation Model},
volume = {20},
journal = {Mathematical Models and Methods in Applied Sciences},
doi = {10.1142/S021820251000443X}
}

@article{dopezu,
author = {Doumic, Marie and Perthame, Benoit and Zubelli, Jorge},
year = {2009},
month = {04},
pages = {045008},
title = {Numerical Solution of an Inverse Problem in Size-Structured Population Dynamics,},
volume = {25},
journal = {Inverse Problems},
doi = {10.1088/0266-5611/25/4/045008}
}

@article{bodoes,
author = {Bourgeron, Thibault and Doumic, Marie and Escobedo, Miguel},
year = {2014},
month = {01},
pages = {},
title = {Estimating the Division Rate of the Self-Similar Growth-Fragmentation Equation},
volume = {30},
journal = {Inverse Problems},
doi = {10.1088/0266-5611/30/2/025007}
}


@article{domazu,
author = {Doumic, Marie and Maia, Pedro and Zubelli, Jorge},
year = {2010},
month = {12},
pages = {405-13},
title = {On the Calibration of a Size-Structured Population Model from Experimental Data},
volume = {58},
journal = {Acta biotheoretica},
doi = {10.1007/s10441-010-9114-9}
}













@article{SLEIJPEN20101100,
title = {Bi-CGSTAB as an induced dimension reduction method},
journal = {Applied Numerical Mathematics},
volume = {60},
number = {11},
pages = {1100-1114},
year = {2010},
note = {Special Issue: 9th IMACS International Symposium on Iterative Methods in Scientific Computing (IISIMSC 2008)},
issn = {0168-9274},
doi = {https://doi.org/10.1016/j.apnum.2009.07.001},
url = {https://www.sciencedirect.com/science/article/pii/S0168927409001238},
author = {G. Sleijpen and P. Sonneveld and M. {van Gijzen}},
keywords = {Bi-CGSTAB, Bi-CG, Iterative linear solvers, Krylov subspace methods, IDR},
abstract = {The Induced Dimension Reduction method [P. Wesseling, P. Sonneveld, Numerical experiments with a multiple grid- and a preconditioned Lanczos type method, in: Lecture Notes in Mathematics, vol. 771, Springer-Verlag, Berlin, 1980, pp. 543–562] was proposed in 1980 as an iterative method for solving large nonsymmetric linear systems of equations. IDR can be considered as the predecessor of methods like CGS (Conjugate Gradient Squared) [P. Sonneveld, CGS, a fast Lanczos-type solver for nonsymmetric linear systems, SIAM J. Sci. Statist. Comput. 10 (1989) 36–52] and Bi-CGSTAB (Bi-Conjugate Gradients STABilized [H.A. van der Vorst, Bi-CGSTAB: A fast and smoothly converging variant of Bi-CG for the solution of nonsymmetric linear systems, SIAM J. Sci. Statist. Comput. 13 (2) (1992) 631–644]). All three methods are based on efficient short recurrences. An important similarity between the methods is that they use orthogonalizations with respect to a fixed ‘shadow residual’. Of the three methods, Bi-CGSTAB has gained the most popularity, and is probably still the most widely used short recurrence method for solving nonsymmetric systems. Recently, Sonneveld and van Gijzen revived the interest for IDR. In [P. Sonneveld, M. van Gijzen, IDR(s): a family of simple and fast algorithms for solving large nonsymmetric systems of linear equations, Preprint, Delft Institute of Applied Mathematics, Delft University of Technology, Delft, The Netherlands, March 2007], they demonstrate that a higher dimensional shadow space, defined by the n×s matrix R˜0, can easily be incorporated into IDR, yielding a highly effective method. The original IDR method is closely related to Bi-CGSTAB. It is therefore natural to ask whether Bi-CGSTAB can be extended in a way similar to IDR. To answer this question we explore the relation between IDR and Bi-CGSTAB and use our findings to derive a variant of Bi-CGSTAB that uses a higher dimensional shadow space.}
}







@article{WU2021101,
title = {A randomized exponential canonical correlation analysis method for data analysis and dimensionality reduction},
journal = {Applied Numerical Mathematics},
volume = {164},
pages = {101-124},
year = {2021},
note = {Special Issue on The Seventh International Conference on Numerical Algebra and Scientific Computing},
issn = {0168-9274},
doi = {https://doi.org/10.1016/j.apnum.2020.09.013},
url = {https://www.sciencedirect.com/science/article/pii/S0168927420302890},
author = {G.Wu and F. Li},
keywords = {Canonical correlation analysis (CCA), Matrix exponential, Randomized singular value decomposition (RSVD), Exponential canonical correlation analysis (ECCA), Generalized eigenvalue problem},
abstract = {Canonical correlation analysis (CCA) is a famous data analysis method that has been successfully used in many areas. CCA extracts meaningful information from a pair of data sets, by seeking pairs of linear combinations from two sets of variables with maximum correlation. Mathematically, CCA resorts to solving a large-scale generalized eigenvalue problem. However, as the dimension of the data sets is much larger than the number of samples, CCA may suffer from the small-sample-size (SSS) problem and the over-fitting problem. In order to overcome these difficulties, the regularized technique is often applied, but it is difficult to choose the optimal parameter in advance. In this work, we propose an Exponential Canonical Correlation Analysis (ECCA) method based on matrix exponential, which is parameter-free and can overcome the over-fitting and the SSS problems fundamentally. However, the computational overhead of the ECCA method is very high in practice. Based on the randomized singular value decomposition (RSVD), we then propose a Randomized Exponential Canonical Correlation Analysis (RECCA) method for data analysis and dimensionality reduction. Theoretical results are given to show the rationality of this randomized method, and establish the relationship between RECCA and ECCA. Numerical experiments are performed on some real-world, high-dimensional and large-sample data sets, which illustrate the superiority of the proposed algorithms over many state-of-the-art CCA algorithms.}
}





@article{SALHOV2015399,
title = "Approximately-isometric diffusion maps",
journal = "Applied and Computational Harmonic Analysis",
volume = "38",
number = "3",
pages = "399 - 419",
year = "2015",
issn = "1063-5203",
doi = "https://doi.org/10.1016/j.acha.2014.05.002",
url = "http://www.sciencedirect.com/science/article/pii/S1063520314000803",
author = "M. Salhov and A. Bermanis and G. Wolf and A. Averbuch",
keywords = "Dimensionality reduction, Manifold learning, Kernel PCA, Diffusion maps, Diffusion distance, Distance preservation",
abstract = "Diffusion Maps (DM), and other kernel methods, are utilized for the analysis of high dimensional datasets. The DM method uses a Markovian diffusion process to model and analyze data. A spectral analysis of the DM kernel yields a map of the data into a low dimensional space, where Euclidean distances between the mapped data points represent the diffusion distances between the corresponding high dimensional data points. Many machine learning methods, which are based on the Euclidean metric, can be applied to the mapped data points in order to take advantage of the diffusion relations between them. However, a significant drawback of the DM is the need to apply spectral decomposition to a kernel matrix, which becomes infeasible for large datasets. In this paper, we present an efficient approximation of the DM embedding. The presented approximation algorithm produces a dictionary of data points by identifying a small set of informative representatives. Then, based on this dictionary, the entire dataset is efficiently embedded into a low dimensional space. The Euclidean distances in the resulting embedded space approximate the diffusion distances. The properties of the presented embedding and its relation to DM method are analyzed and demonstrated."
}

@article{MARSHALL2018709,
title = "Time coupled diffusion maps",
journal = "Applied and Computational Harmonic Analysis",
volume = "45",
number = "3",
pages = "709 - 728",
year = "2018",
issn = "1063-5203",
doi = "https://doi.org/10.1016/j.acha.2017.11.003",
url = "http://www.sciencedirect.com/science/article/pii/S1063520317301276",
author = "N. F. Marshall and M. J. Hirn",
keywords = "Manifold learning, Dimensionality reduction, Diffusion distance, Heat equation, Time-dependent metric",
abstract = "We consider a collection of n points in Rd measured at m times, which are encoded in an n×d×m data tensor. Our objective is to define a single embedding of the n points into Euclidean space which summarizes the geometry as described by the data tensor. In the case of a fixed data set, diffusion maps and related graph Laplacian methods define such an embedding via the eigenfunctions of a diffusion operator constructed on the data. Given a sequence of m measurements of n points, we introduce the notion of time coupled diffusion maps which have natural geometric and probabilistic interpretations. To frame our method in the context of manifold learning, we model evolving data as samples from an underlying manifold with a time-dependent metric, and we describe a connection of our method to the heat equation on such a manifold."
}






@article {Coifman7426,
	author = {Coifman, R. R. and Lafon, S. and Lee, A. B. and Maggioni, M. and Nadler, B. and Warner, F. and Zucker, S. W.},
	title = {Geometric diffusions as a tool for harmonic analysis and structure definition of data: Diffusion maps},
	volume = {102},
	number = {21},
	pages = {7426--7431},
	year = {2005},
	doi = {10.1073/pnas.0500334102},
	publisher = {National Academy of Sciences},
	abstract = {We provide a framework for structural multiscale geometric organization of graphs and subsets of \mathbb{R}^{n}. We use diffusion semigroups to generate multiscale geometries in order to organize and represent complex structures. We show that appropriately selected eigenfunctions or scaling functions of Markov matrices, which describe local transitions, lead to macroscopic descriptions at different scales. The process of iterating or diffusing the Markov matrix is seen as a generalization of some aspects of the Newtonian paradigm, in which local infinitesimal transitions of a system lead to global macroscopic descriptions by integration. We provide a unified view of ideas from data analysis, machine learning, and numerical analysis.},
	issn = {0027-8424},
	URL = {https://www.pnas.org/content/102/21/7426},
	eprint = {https://www.pnas.org/content/102/21/7426.full.pdf},
	journal = {Proceedings of the National Academy of Sciences}
}




@article{DAS2004715,
title = "The {L}aplacian spectrum of a graph",
journal = "Computers $\&$ Mathematics with Applications",
volume = "48",
number = "5",
pages = "715 - 724",
year = "2004",
issn = "0898-1221",
doi = "https://doi.org/10.1016/j.camwa.2004.05.005",
url = "http://www.sciencedirect.com/science/article/pii/S0898122104003074",
author = "K. Ch. Das",
keywords = "Graph, Laplacian matrix, Largest eigenvalue, Upper bound",
abstract = "Let G = (V, E) be a simple graph. Denote by D(G) the diagonal matrix of its vertexdegrees and by A(G) its adjacency matrix. Then, the Laplacian matrix of G is L(G) = D(G) − A(G). The first and second section of this paper contains introduction and some known results, respectively. The third section is devoted to properties of Laplacian spectrum. The fourth section contains characterization of graphs. The fifth section relates the Laplacian eigenvalues with the graph structure."
}

@ARTICLE{6789755,
author={M. {Belkin} and P. {Niyogi}},
journal={Neural Computation},
title={Laplacian Eigenmaps for Dimensionality Reduction and Data Representation},
year={2003},
volume={15},
number={6},
pages={1373-1396},
keywords={},
doi={10.1162/089976603321780317},
ISSN={0899-7667},
month={June},}

@article{HAJJI20041011,
title = "Representation of differential operators in wavelet basis",
journal = "Computers $\&$  Mathematics with Applications",
volume = "47",
number = "6",
pages = "1011 - 1033",
year = "2004",
issn = "0898-1221",
doi = "https://doi.org/10.1016/S0898-1221(04)90083-1",
url = "http://www.sciencedirect.com/science/article/pii/S0898122104900831",
author = "M.A Hajji and S Melkonian and R Vaillancourt",
keywords = "Wavelet, Partial-differential operator, Circulant, Block circulant",
abstract = "Existing work on the representation of operators in one-dimensional, compactly-supported, orthonormal wavelet bases is extended to two dimensions. The nonstandard form of the representation of operators is given in separable two-dimensional, periodic, orthonormal wavelet bases. The matrix representation of the partial-differential operators ∂x and ∂y are constructed and a closed form formula for the matrix representation of a general partial-differential operator g(∂x, ∂y) is derived, where g is an analytic function."
}

@book{functio,
  title={ Functional Analysis in Applied Mathematics and Engineering},
  author={M. Pedersen},
  year={1999},
  publisher={CRC Press}
}



@article{Alzubi_2018,
	doi = {10.1088/1742-6596/1142/1/012012},
	url = {https://doi.org/10.1088%2F1742-6596%2F1142%2F1%2F012012},
	year = 2018,
	month = {nov},
	publisher = {{IOP} Publishing},
	volume = {1142},
	pages = {012012},
	author = {J. Alzubi and A. Nayyar and A. Kumar},
	title = {Machine Learning from Theory to Algorithms: An Overview},
	journal = {Journal of Physics: Conference Series},
	abstract = {The current SMAC (Social, Mobile, Analytic, Cloud) technology trend paves the way to a future in which intelligent machines, networked processes and big data are brought together. This virtual world has generated vast amount of data which is accelerating the adoption of machine learning solutions $\&$  practices. Machine Learning enables computers to imitate and adapt human-like behaviour. Using machine learning, each interaction, each action performed, becomes something the system can learn and use as experience for the next time. This work is an overview of this data analytics method which enables computers to learn and do what comes naturally to humans, i.e. learn from experience. It includes the preliminaries of machine learning, the definition, nomenclature and applications’ describing it’s what, how and why. The technology roadmap of machine learning is discussed to understand and verify its potential as a market $\&$  industry practice. The primary intent of this work is to give insight into why machine learning is the future.}
}

@misc{acuepar,
  title = {{The Paris Agreement}},
  howpublished = {\url{https://unfccc.int/process-and-meetings/the-paris-agreement/d2hhdC1pcy}},
    author={United Nations Framework Convention on Climate Change},
  note = {Accessed: 2020-06-01}
}




@article{climacamb,
author = {Hansen, J. and Ruedy, R. and Sato, M. and Lo, K.},
title = {GLOBAL SURFACE TEMPERATURE CHANGE},
journal = {Reviews of Geophysics},
volume = {48},
number = {4},
pages = {},
keywords = {global temperature, temperature analysis, climate change, global change, El Niño-La Niña},
doi = {10.1029/2010RG000345},
url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1029/2010RG000345},
eprint = {https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1029/2010RG000345},
abstract = {We update the Goddard Institute for Space Studies (GISS) analysis of global surface temperature change, compare alternative analyses, and address questions about perception and reality of global warming. Satellite-observed night lights are used to identify measurement stations located in extreme darkness and adjust temperature trends of urban and periurban stations for nonclimatic factors, verifying that urban effects on analyzed global change are small. Because the GISS analysis combines available sea surface temperature records with meteorological station measurements, we test alternative choices for the ocean data, showing that global temperature change is sensitive to estimated temperature change in polar regions where observations are limited. We use simple 12 month (and n × 12) running means to improve the information content in our temperature graphs. Contrary to a popular misconception, the rate of warming has not declined. Global temperature is rising as fast in the past decade as in the prior 2 decades, despite year-to-year fluctuations associated with the El Niño-La Niña cycle of tropical ocean temperature. Record high global 12 month running mean temperature for the period with instrumental data was reached in 2010.},
year = {2010}
}

@misc{climacamb1,
  title = {{World of Change: Global Temperatures}},
  howpublished = {\url{https://earthobservatory.nasa.gov/world-of-change/DecadalTemp}},
    author={Earth observatory},
  note = {Accessed: 2020-06-01}
}

@misc{Tomjo,
  title = {{Tom Jobim in Ipanema Beach picture}},
  howpublished = {\url{https://www.diariodecultura.com.ar/columnas/crucigrama-antonio-brasileiro/}},
    author={Diario de cultura},
  note = {Accessed: 2020-06-01}
}

@misc{climain,
  title = {{Brazilian temperature dataset}},
  howpublished = {\url{http://www.inmet.gov.br/portal/}},
    author={INMET},
  note = {Accessed: 2020-06-01}
}

 
@book{grafakos2014classical,
  title={Classical Fourier Analysis},
  author={Grafakos, L.},
  series={Graduate Texts in Mathematics},
  year={2014},
  publisher={Springer New York}
}

@book{steinsingu,
 author = {E. M. Stein},
 publisher = {Princeton University Press},
 title = {Singular Integrals and Differentiability Properties of Functions},
 year = {1970}
}

@article{COIFMAN20065,
title = "Diffusion maps",
journal = "Applied and Computational Harmonic Analysis",
volume = "21",
number = "1",
pages = "5 - 30",
year = "2006",
note = "Special Issue: Diffusion Maps and Wavelets",
issn = "1063-5203",
doi = "https://doi.org/10.1016/j.acha.2006.04.006",
url = "http://www.sciencedirect.com/science/article/pii/S1063520306000546",
author = "R.  R. Coifman and S. Lafon",
keywords = "Diffusion processes, Diffusion metric, Manifold learning, Dimensionality reduction, Eigenmaps, Graph Laplacian",
abstract = "In this paper, we provide a framework based upon diffusion processes for finding meaningful geometric descriptions of data sets. We show that eigenfunctions of Markov matrices can be used to construct coordinates called diffusion maps that generate efficient representations of complex geometric structures. The associated family of diffusion distances, obtained by iterating the Markov matrix, defines multiscale geometries that prove to be useful in the context of data parametrization and dimensionality reduction. The proposed framework relates the spectral properties of Markov processes to their geometric counterparts and it unifies ideas arising in a variety of contexts such as machine learning, spectral graph theory and eigenmap methods."
}

@article{COIFMAN201479,
title = "Diffusion maps for changing data",
journal = "Applied and Computational Harmonic Analysis",
volume = "36",
number = "1",
pages = "79 - 107",
year = "2014",
issn = "1063-5203",
doi = "https://doi.org/10.1016/j.acha.2013.03.001",
url = "http://www.sciencedirect.com/science/article/pii/S1063520313000225",
author = "R. R. Coifman and M. J. Hirn",
keywords = "Diffusion distance, Graph Laplacian, Manifold learning, Dynamic graphs, Dimensionality reduction, Kernel method, Spectral graph theory",
abstract = "Graph Laplacians and related nonlinear mappings into low dimensional spaces have been shown to be powerful tools for organizing high dimensional data. Here we consider a data set X in which the graph associated with it changes depending on some set of parameters. We analyze this type of data in terms of the diffusion distance and the corresponding diffusion map. As the data changes over the parameter space, the low dimensional embedding changes as well. We give a way to go between these embeddings, and furthermore, map them all into a common space, allowing one to track the evolution of X in its intrinsic geometry. A global diffusion distance is also defined, which gives a measure of the global behavior of the data over the parameter space. Approximation theorems in terms of randomly sampled data are presented, as are potential applications."
}

@article{SALHOV2018324,
title = "Diffusion representations",
journal = "Applied and Computational Harmonic Analysis",
volume = "45",
number = "2",
pages = "324 - 340",
year = "2018",
issn = "1063-5203",
doi = "https://doi.org/10.1016/j.acha.2016.10.003",
url = "http://www.sciencedirect.com/science/article/pii/S1063520316300690",
author = "M. Salhov and A. Bermanis and G. Wolf and A. Averbuch",
keywords = "Manifold learning, Kernel PCA, Diffusion Maps, Diffusion distance, Distance preservation",
abstract = "Diffusion Maps framework is a kernel based method for manifold learning and data analysis that defines diffusion similarities by imposing a Markovian process on the given dataset. Analysis by this process uncovers the intrinsic geometric structures in the data. Recently, it was suggested to replace the standard kernel by a measure-based kernel that incorporates information about the density of the data. Thus, the manifold assumption is replaced by a more general measure-based assumption. The measure-based diffusion kernel incorporates two separate independent representations. The first determines a measure that correlates with a density that represents normal behaviors and patterns in the data. The second consists of the analyzed multidimensional data points. In this paper, we present a representation framework for data analysis of datasets that is based on a closed-form decomposition of the measure-based kernel. The proposed representation preserves pairwise diffusion distances that does not depend on the data size while being invariant to scale. For a stationary data, no out-of-sample extension is needed for embedding newly arrived data points in the representation space. Several aspects of the presented methodology are demonstrated on analytically generated data."
}


@book{engl1996regularization,
  title={Regularization of Inverse Problems},
  author={Engl, H.W. and Hanke, M. and Neubauer, A.},
  isbn={9780792341574},
  lccn={lc96028672},
  series={Mathematics and Its Applications},
  url={https://books.google.com.co/books?id=2bzgmMv5EVcC},
  year={1996},
  publisher={Springer Netherlands}
}





















@INPROCEEDINGS{india,  
author={Malhotra, E. and Rajwade, A.}, 
booktitle={2016 IEEE International Conference on Image Processing (ICIP)},   title={Tomographic reconstruction from projections with unknown view angles exploiting moment-based relationships},
year={2016},  
volume={},  
number={}, 
pages={1759-1763}, 
doi={10.1109/ICIP.2016.7532660}}


@INPROCEEDINGS{angudesco,
  author={Basu, S. and Bresler, Y.},
  booktitle={Proceedings 1998 International Conference on Image Processing. ICIP98}, 
  title={Feasibility of tomography with unknown view angles}, 
  year={1998},
  pages={15-19 vol.2},
  }



@misc{radiografi,
  title = {{Tomographic image of a knee}},
  howpublished = {\url{https://radiopaedia.org/cases/normal-ct-knee-1}},
    author={J.Cheng},
  note = {Accessed: 2021-11-01}
}



@ARTICLE{angucoif,
  author={Coifman, R. and Shkolnisky, Y. and Sigworth, F. and Singer, A.},
  journal={IEEE Transactions on Image Processing}, 
  title={Graph Laplacian Tomography From Unknown Random Projections}, 
  year={2008},
  volume={17},
  number={10},
  pages={1891-1899},
  doi={10.1109/TIP.2008.2002305}}


@book{radon3,
  title={Fundamentals of Computerized Tomography: Image Reconstruction from Projections},
  author={Herman, G.T.},
  isbn={9781846287237},
  lccn={2009929054},
  series={Advances in Computer Vision and Pattern Recognition},
  url={https://books.google.ae/books?id=BhtGTkEjkOQC},
  year={2009},
  publisher={Springer London}
}




@book{radon2,
author = {Kak, A. and Slaney, M.},
title = {Principles of Computerized Tomographic Imaging},
publisher = {Society for Industrial and Applied Mathematics},
year = {2001},
doi = {10.1137/1.9780898719277},
address = {},
edition   = {},
URL = {https://epubs.siam.org/doi/abs/10.1137/1.9780898719277},
eprint = {https://epubs.siam.org/doi/pdf/10.1137/1.9780898719277}
}


@book{radon1,
  title={The Radon Transform and Some of Its Applications},
  author={Deans, S.R.},
  isbn={9780471898047},
  lccn={83001125},
  series={A Wiley-Interscience publication},
  url={https://books.google.ae/books?id=kVTvAAAAMAAJ},
  year={1983},
  publisher={Wiley}
}



@article{learning2,
author = {Mukherjee, S. and Wu, Q.},
year = {2006},
month = {12},
pages = {2481-2514},
title = {Estimation of Gradients and Coordinate Covariation in Classification},
volume = {7},
journal = {Journal of Machine Learning Research}
}


@article{gradteo2,
author = {Daubechies, I. and Teschke, G. and Vese, L.},
year = {2007},
month = {02},
pages = {29-46},
title = {Iteratively solving linear inverse problems under general convex constraints},
volume = {1},
journal = {Inverse Problems and Imaging},
doi = {10.3934/ipi.2007.1.29}
}


  @manual{alvarorepo,
      title  = "Codes and numerical implementations of this thesis",
      author = "A. Gomez",
      note   = "\url{https://github.com/zabu182}",
      year   = "Dec. 1, 2021 "
    }



  @manual{manopt2,
      title  = "Manopt Toolbox",
      author = "N. Boumal and B. Mishra",
      note   = "\url{https://github.com/NicolasBoumal/manopt}",
      year   = "Sep. 5, 2021 "
    }





@article{manopt1,
  author  = {N. Boumal and B. Mishra and P.-A. Absil and R. Sepulchre},
  title   = {Manopt, a Matlab Toolbox for Optimization on Manifolds},
  journal = {Journal of Machine Learning Research},
  year    = {2014},
  volume  = {15},
  number  = {42},
  pages   = {1455-1459},
  url     = {http://jmlr.org/papers/v15/boumal14a.html}
}







@book{spheregrassmanian,
  title={Lagrangian and Hamiltonian Methods For Nonlinear Control 2006: Proceedings from the 3rd IFAC Workshop, Nagoya, Japan, July 2006},
  author={Bullo, F. and Fujimoto, K.},
  isbn={9783540738909},
  series={Lecture Notes in Control and Information Sciences},
  year={2007},
  publisher={Springer Berlin Heidelberg}
}



@article{gradientgrafo,
author = {Bensoussan, A. and Menaldi, J.},
year = {2003},
pages = {},
title = {Difference equations on weighted graphs},
volume = {12},
journal = {Journal of Convex Analysis}
}




@article{denoising,
author = {Bresson, X. and Chan, T.},
year = {2008},
month = {11},
pages = {455-484},
title = {Fast dual minimization of the vectorial total variation norm and applications to color image processing},
volume = {2},
journal = {Inverse Problems and Imaging},
doi = {10.3934/ipi.2008.2.455}
}





@book{sepul,
author = {Absil, P. and Mahony, R. and Sepulchre, R.},
year = {2008},
title = {Optimization Algorithms on Matrix Manifolds},
volume = {78},
isbn = {978-0-691-13298-3},
journal = {Mathematics of Computation - Math. Comput.},
publisher = {Princenton University Press},
doi = {10.1515/9781400830244}
}







@article{ZMSG2003,
	doi = {10.1088/0266-5611/19/4/310},
	url = {https://doi.org/10.1088/0266-5611/19/4/310},
	year = 2003,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {19},
	number = {4},
	pages = {933--949},
	author = {J P Zubelli and R Marabini and C O S Sorzano and G T Herman},
	title = {Three-dimensional reconstruction by {Chahine's} method from electron microscopic projections corrupted by instrumental aberrations},
	journal = {Inverse Problems},
	abstract = {Three-dimensional reconstruction of nano-scale objects (such as biological macromolecules) can be accomplished using data recorded with a transmission electron microscope. An image obtained by a transmission electron microscope can be conceived of as an ‘ideal’ projection subjected to a contrast transfer function, which attenuates most frequencies, reverses the phase of others and even eliminates some of them. Such instrumental aberrations make the problem of reconstruction from such data difficult. We reformulate the problem so that Chahine’s method becomes applicable to it. We demonstrate the performance of our approach with numerical evidence using both simulated and actual electron microscopy data.}
}

@article{PWD2020,
title = {Manifold learning for accelerating coarse-grained optimization},
journal = {Journal of Computational Dynamics},
volume = {7},
number = {2},
pages = {511-536},
year = {2020},
author = {D. Pozharskiy and N. Wichrowski and Andrew B. Duncan and  Grigorios A. Pavliotis and  Ioannis G. Kevrekidis}
}

@Article{MZ2001,
	AUTHOR = "G. Malajovich and J. P. Zubelli",
	TITLE = "On the Geometry of Graeffe Iteration",
	JOURNAL = "Journal of Complexity",
	VOLUME = "17",
	YEAR = "2001",
	NUMBER = "3",
	PAGES = "541--573"
}

@Article{MR2002m,
	AUTHOR = "G. Malajovich and J. P. Zubelli",
	TITLE = "Tangent Graeffe Iteration. ",
	JOURNAL = "Numerische Mathematik",
	VOLUME = "89",
	YEAR = "2001",
	NUMBER = "4",
	PAGES = "749--782"
}

@article{alvaro,
title = {Diffusion representation for asymmetric kernels},
journal = {Applied Numerical Mathematics},
volume = {166},
pages = {208-226},
year = {2021},
issn = {0168-9274},
doi = {https://doi.org/10.1016/j.apnum.2021.04.002},
url = {https://www.sciencedirect.com/science/article/pii/S016892742100101X},
author = {A. {Almeida Gomez} and A. {Silva Neto} and J. Zubelli},
keywords = {Diffusion maps, Dimensional reduction, FFT, Asymmetric kernels},
abstract = {We extend the diffusion-map formalism to data sets that are induced by asymmetric kernels. Analytical convergence results of the resulting expansion are proved, and an algorithm is proposed to perform the dimensional reduction. A coordinate system connected to the tensor product of Fourier basis is used to represent the underlying geometric structure obtained by the diffusion-map, thus reducing the dimensionality of the data set and making use of the speedup provided by the two-dimensional Fast Fourier Transform algorithm (2-D FFT). We compare our results with those obtained by other eigenvalue expansions, and verify the efficiency of the algorithms with synthetic data, as well as with real data from applications including climate change studies.}
}


@article{cressey_cryo-electron_2017,
	title = {Cryo-electron microscopy wins chemistry {Nobel}},
	volume = {550},
	issn = {0028-0836, 1476-4687},
	url = {http://www.nature.com/articles/nature.2017.22738},
	doi = {10.1038/nature.2017.22738},
	language = {en},
	number = {7675},
	urldate = {2021-04-01},
	journal = {Nature},
	author = {Cressey, D. and Callaway, E.},
	month = oct,
	year = {2017},
	pages = {167--167},
}

@article{SINGER2010312,
author = {Singer, A. and Coifman, R. and Sigworth, F. and Chester, D. and Shkolnisky, Yoel},
year = {2009},
month = {11},
pages = {312-22},
title = {Detecting Consistent Common Lines in Cryo-EM by Voting},
volume = {169},
journal = {Journal of structural biology},
doi = {10.1016/j.jsb.2009.11.003}
}



@article{henderson_three-dimensional_1975,
author = {Henderson, R. and Unwin, P.N.T.},
year = {1975},
month = {10},
pages = {28-32},
title = {Henderson, R.  Unwin, P. N. T. Three-dimensional model of purple membrane obtained by electron microscopy. Nature 257, 28-32},
volume = {257},
journal = {Nature},
doi = {10.1038/257028a0}
}



@article{HENDERSON1990899,
author = {Henderson, R.},
year = {1989},
month = {12},
pages = {467-467},
title = {Model for the structure of bacteriorhodopsin based on high-resolution electron cryo-microscopy},
volume = {31},
journal = {Ultramicroscopy},
doi = {10.1016/0304-3991(89)90371-9}
}

@article{singer_three-dimensional_2011,
author = {Singer, A. and Shkolnisky, Y.},
year = {2011},
month = {06},
pages = {543-572},
title = {Three-Dimensional Structure Determination from Common Lines in Cryo-EM by Eigenvectors and Semidefinite Programming},
volume = {4},
journal = {SIAM journal on imaging sciences},
doi = {10.1137/090767777}
}


@article{cryo-em_2018,
author = {Ceska, C. and Cooke, R. and Phillips, C. and Williams, P.},
year = {2019},
month = {01},
pages = {BST20180267},
title = {Cryo-EM in drug discovery},
volume = {47},
journal = {Biochemical Society Transactions},
doi = {10.1042/BST20180267}
}


@article{cryoBAI201549,
author = {Bai, X. and McMullan, G. and Scheres, S.},
year = {2014},
month = {11},
pages = {},
title = {How cryo-EM is revolutionizing structural biology. Trends Biochem},
volume = {40},
journal = {Trends in Biochemical Sciences},
doi = {10.1016/j.tibs.2014.10.005}
}


@article{
Cryo1,
author = {Murata, Kazuyoshi and Wolf, Matthias},
year = {2017},
month = {07},
pages = {},
title = {Cryo-Electron Microscopy for Structural Analysis of Dynamic Biological Macromolecules},
volume = {1862},
journal = {Biochimica et Biophysica Acta (BBA) - General Subjects},
doi = {10.1016/j.bbagen.2017.07.020}
}






@article{libroedo,
author = {Teschl, G.},
year = {2008},
month = {01},
pages = {},
title = {Ordinary differential equations and dynamical systems},
journal = {American Mathematical Society}
}
 
 
 
 
 
 @book{evans10,
  abstract = {"This is the second edition of the now definitive text on partial differential equations (PDE). It offers a comprehensive survey of modern techniques in the theoretical study of PDE with particular emphasis on nonlinear equations. Its wide scope and clear exposition make it a great text for a graduate course in PDE. For this edition, the author has made numerous changes, including: a new chapter on nonlinear wave equations, more than 80 new exercises, several new sections, and a significantly expanded bibliography."--Publisher's description.},
  added-at = {2015-07-29T08:37:26.000+0200},
  address = {Providence, R.I.},
  author = {Evans, L.},
  biburl = {https://www.bibsonomy.org/bibtex/2f5b120723ea78913e7e700ddd1a99301/ytyoun},
  interhash = {59982ce44cc43813ccb14c0d647a59ee},
  intrahash = {f5b120723ea78913e7e700ddd1a99301},
  isbn = {9780821849743 0821849743},
  keywords = {partial.differential.equations pde textbook},
  publisher = {American Mathematical Society},
  refid = {465190110},
  timestamp = {2015-07-29T08:37:26.000+0200},
  title = {Partial differential equations},
  year = 2010
}


 
 
  @article{schnorr1994lattice,
  title={Lattice basis reduction: Improved practical algorithms and solving subset sum problems},
  author={Schnorr, C. and Euchner, M.},
  journal={Mathematical programming},
  volume={66},
  number={1-3},
  pages={181--199},
  year={1994},
  publisher={Springer}
}
 
 
 
  @manual{softwa,
      title  = "Implementation of shortest vector of a lattice using exhaustive enumeration",
      author = "C. Chapman",
      note   = "\url{https://github.com/enthdegree/lenum.m}",
      year   = "2018 (accessed December 1, 2021)"
    }
  


@article{Groemer1963,
author = {Groemer, H.},
year = {1968},
month = {08},
pages = {325-334},
title = {Existenzsätze für Lagerungen in metrischen Räumen},
volume = {72},
journal = {Monatshefte Fur Mathematik},
doi = {10.1007/BF01302167}
}




@article{mari245,
author = {Cohn, H. and Kumar, A. and Miller, S. and Radchenko, D. and Viazovska, M.},
year = {2016},
month = {03},
pages = {},
title = {The sphere packing problem in dimension 24},
volume = {185},
journal = {Annals of Mathematics},
doi = {10.4007/annals.2017.185.3.8}
}



@article{mari8,
author = {Viazovska, M.},
year = {2016},
month = {03},
pages = {},
title = {The sphere packing problem in dimension 8},
volume = {185},
journal = {Annals of Mathematics},
doi = {10.4007/annals.2017.185.3.7}
}





@article{10.2307/20159940,
 ISSN = {0003486X},
 URL = {http://www.jstor.org/stable/20159940},
 author = {T. Hales},
 journal = {Annals of Mathematics},
 number = {3},
 pages = {1065--1185},
 publisher = {Annals of Mathematics},
 title = {A Proof of the Kepler Conjecture},
 volume = {162},
 year = {2005}
}

@article{articlegradient,
author = {Tripuraneni, Nilesh and Flammarion, Nicolas and Bach, Francis and Jordan, Michael},
year = {2018},
month = {02},
pages = {},
title = {Averaging Stochastic Gradient Descent on Riemannian Manifolds},
journal = {Proceedings of the 31st  Conference On Learning Theory}
}




@book{do1992riemannian,
  title={Riemannian Geometry},
  author={do Carmo, M.},
  isbn={9783764334901},
  lccn={91037377},
  series={Mathematics (Boston, Mass.)},
  url={https://books.google.com.co/books?id=uXJQQgAACAAJ},
  year={1992},
  publisher={Birkh{\"a}user}
}













@book{claudia,
author = {Bonnans, J. and Gilbert, J. and Lemaréchal, C and Sagastizabal, C.},
year = {2006},
month = {01},
pages = {},
title = {Numerical Optimization -- Theoretical and Practical Aspects},
journal = {Springer},
publisher  = {Springer}
}


@article{6487381,
author = {Bonnabel, Silvère},
year = {2011},
month = {11},
pages = {},
title = {Stochastic Gradient Descent on Riemannian Manifolds},
volume = {58},
journal = {IEEE Transactions on Automatic Control},
doi = {10.1109/TAC.2013.2254619}
}


  
 





@article{paperfundamental,
author = {Berahas, A. and Cao, L. and Choromanski, K.f and Scheinberg, K.},
year = {2021},
month = {05},
title = {A Theoretical and Empirical Comparison of Gradient Approximations in Derivative-Free Optimization},
journal = {Foundations of Computational Mathematics},
}
